Learning to Estimate System Specifications in Linear Temporal Logic using Transformers and Mamba

Temporal logic is a framework for representing and reasoning about propositions that evolve over time. It is commonly used for specifying requirements in various domains, including hardware and software systems, as well as robotics. Specification mining or formula generation involves extracting temporal logic formulae from system traces and has numerous applications, such as detecting bugs and improving interpretability. Although there has been a surge of deep learning-based methods for temporal logic satisfiability checking in recent years, the specification mining literature has been lagging behind in adopting deep learning methods despite their many advantages, such as scalability. In this paper, we introduce autoregressive models that can generate linear temporal logic formulae from traces, towards addressing the specification mining problem. We propose multiple architectures for this task: transformer encoder-decoder, decoder-only transformer, and Mamba, which is an emerging alternative to transformer models. Additionally, we devise a metric for quantifying the distinctiveness of the generated formulae and a straightforward algorithm to enforce the syntax constraints. Our experiments show that the proposed architectures yield promising results, generating correct and distinct formulae at a fraction of the compute cost needed for the combinatorial baseline.

==> sections/table_all_v0.tex <==
\begin{table}[htbp]
  \caption{
    Average test set evaluation of all architectures.
    The best performing model for each architecture was trained three times from scratch and evaluated.
    Average and standard deviation of these results are reported.
  }
  \label{test-set-mean}
  \centering
    { % \small %
  \begin{tabular}{lrrrrr}
    \toprule
    Architecture &  Correct $\%$ & Exact $\%$ & Incorrect $\%$ & Invalid $\%$ & Timeout $\%$ \\
    \midrule
    Transformer  & $94.38 \pm 4.12$ & $1.00 \pm 0.02$ & $4.45 \pm 3.68$ & $0.03 \pm 0.02$ & $1.14 \pm 0.50$ \\
    Mamba        & $98.23 \pm 0.29$ & $0.98 \pm 0.01$ & $1.38 \pm 0.11$ & $0.00 \pm 0.00$ & $0.39 \pm 0.18$ \\
    Llama        & $95.75 \pm 2.09$ & $0.93 \pm 0.01$ & $1.98 \pm 0.87$ & $0.00 \pm 0.00$ & $2.26 \pm 2.06$ \\
    \bottomrule
  \end{tabular} }
\end{table}

\begin{table}[htbp]
  \caption{
    Example trace-formula pairs from the LTLRandom35's test set and the models' predictions.
    The predictions in this table are unanimous, i.e., all 9 models considered in Table~\ref{test-set-mean} made the same prediction.
  }
  \label{example-unanimous}
  \centering
 %   \resizebox{0.9\linewidth}{!}{
    { % \small
  \begin{tabular}{ccc}
    \toprule
    Trace & Ground Truth & Prediction \\
    \midrule
    $1, b, d \wedge e, c, (1)^\omega$  % index 0
    & $\X (\neg (b \wedge  \neg \X e) \wedge  \X \X c \until  \X ((\neg d \until  d) \until  \X c))$
    & $\X (b \wedge  \X (d \wedge  e \wedge  \X c))$
    \\
    $b \wedge  \neg d, (b)^\omega$ % SAMPLE 199
    & $\neg d \wedge  \neg (1 \until  \neg b \wedge  \X ((1 \until  \neg c) \until  d \until  a))$
    & $\neg d \wedge  \neg (1 \until  \neg b)$
    \\
    $a \wedge  \neg e, e, d, (1)^\omega$ % index 176
    & $a \until  e \wedge  \X \X d$
    & $a \until  e \wedge  \X \X d$
    \\
    \bottomrule
  \end{tabular} }
\end{table}

\begin{table}[htbp]
  \caption{
    Examples of semantically correct formula predictions for the trace samples from the LTLRandom35's test set.
  }
  \label{example2}
  \centering
    { %\small
  \begin{tabular}{ccc}
    \toprule
    Trace & Formula & Source \\
    \midrule
    \multirow{3}{*}{$1, a \wedge  \neg c \wedge  \neg e, (a)^\omega$} % index 10
    & $\X (\neg c \wedge  \neg e \wedge  \neg (1 \until  \neg a))$ & Transformer A, B, C; Mamba A \\
    & $\X \neg (1 \until  \neg a) \wedge  \X (\neg c \wedge  \neg e)$ & Mamba B \\
    & $\X (\neg c \wedge  \neg e \wedge  \neg (1 \until  \neg a))$ & Mamba C; Llama A, B, C \\
    \midrule
    \multirow{2}{*}{$1, \neg b, (1)^\omega$} % index 2
    & $(\neg b \wedge  c) \until  \neg \X (b \wedge  \X d)$ & Ground Truth \\
    & $\neg (\X b \wedge  \X^{30} a)$ & Transformer A \\
    \midrule
    $1, b, e, (1)^\omega$ % index 4
    & $\X b \wedge  \X \X (\neg \X^{25} b \until  e)$ & Llama B \\
    \bottomrule
  \end{tabular} }
\end{table}


\begin{table}[htbp]
  \caption{
    Formula predictions for the various traces from the LTLRandom35's test set.
    The first trace is $\neg c, \neg c \wedge  \neg d, c \wedge  \neg d, \neg b, \neg b, (1)^\omega$,
    the second one is $1, 1, c, (1)^\omega$.
    In the source column, we merged the predictions that were syntactically different but semantically equivalent.
  }
  \label{example-mixed}
  \centering
    { %\small
  \begin{tabular}{cccc}
    \toprule
    Trace \# & Formula & Source & Evaluation \\
    \midrule
    \multirow{2}{*}{1} % index 150
    & $\neg (\neg c \until  \X d) \wedge  \X \X \X \neg (\X b \until  b)$ & Transformer C; Mamba A, B & Incorrect \\
    & $\X \neg d \until  c \wedge  \neg \X \X \X (\X b \until  b)$ & Transformer A, B & Correct \\
    \midrule
    \multirow{2}{*}{2} % index 213
    & $\X \X (\X^{30} c \until \X c)$ & Transformer B & Incorrect \\
    & $\X \X (\X^{25} \neg a \until  c)$ & Mamba A & Correct \\
    \bottomrule
  \end{tabular} }
\end{table}



==> sections/table_all_v1_cancelled.tex <==
\begin{table}[htbp]
  \caption{
    Example trace-formula pairs from the LTLRandom35's test set and the models' predictions.
  }
  \label{example-unanimous}
  \centering
    \resizebox{1\linewidth}{!}{
    % \small
  \begin{tabular}{cccc}
    \toprule
    Trace & Ground Truth & Prediction & Model \\
    \midrule
      \multirow{2}{*}{$1, b, d \wedge e, c, (1)^\omega$}  % index 0
      & \multirow{2}{*}{\shortstack{$\X (\neg (b \wedge  \neg \X e) \wedge  \X \X c \until$\\$\X ((\neg d \until  d) \until  \X c))$}}
      & \multirow{2}{*}{$\X (b \wedge  \X (d \wedge  e \wedge  \X c))$}
      & \multirow{2}{*}{All models} \\
      & & & \\
    \mytabsep
    $b \wedge  \neg d, (b)^\omega$ % SAMPLE 199
    & $\neg d \wedge  \neg (1 \until  \neg b \wedge  \X ((1 \until  \neg c) \until  d \until  a))$
    & $\neg d \wedge  \neg (1 \until  \neg b)$
    & All models
    \\
    \mytabsep
    $a \wedge  \neg e, e, d, (1)^\omega$ % index 176
    & $a \until  e \wedge  \X \X d$
    & $a \until  e \wedge  \X \X d$
    & All models
    \\
    \mytabsep
    \multirow{3}{*}{$1, a \wedge  \neg c \wedge  \neg e, (a)^\omega$} % index 10
      & \multirow{3}{*}{\shortstack{$(\X (a \wedge  \neg e) \until  1 \until  e) \until$\\$  (\X \neg c \wedge  \X (b \until  \neg e) \wedge$\\$\neg \X (\X c \until  1 \until  \neg a))$}}
      & $\X (\neg c \wedge  \neg e \wedge  \neg (1 \until  \neg a))$ & $\text{Trans}_\text{A,B,C}$; $\text{Mamba}_\text{A}$ \\
      & & $\X \neg (1 \until  \neg a) \wedge  \X (\neg c \wedge  \neg e)$ & $\text{Mamba}_\text{B}$ \\
      & & $\X (\neg c \wedge  \neg e \wedge  \neg (1 \until  \neg a))$ & $\text{Mamba}_\text{C}, \text{Llama}_\text{A,B,C}$ \\
    \bottomrule
  \end{tabular} }
\end{table}

